Two Roads to Classicality

Mixing and decoherence are both manifestations of classicality within quantum theory, each of which admit a very general category-theoretic construction. We show under which conditions these two 'roads to classicality' coincide. This is indeed the case for (finite-dimensional) quantum theory, where each construction yields the category of C*-algebras and completely positive maps. We present counterexamples where the property fails which includes relational and modal theories. Finally, we provide a new interpretation for our category-theoretic generalisation of decoherence in terms of 'leaking information'.

==> eptcsdata.tex <==
\providecommand{\firstpage}{104}
\providecommand{\publicationstatus}{Bob Coecke and Aleks Kissinger (Eds.):\\ 14th International Conference on Quantum Physics and Logic (QPL)\\
EPTCS 266, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.266.7}{10.4204/EPTCS.266.7}}

